A11yLTLNav: Automatic Detection of Accessibility Navigation Failures

For blind and low-vision (BLV) screen-reader users, a website that appears accessible in a static snapshot can become difficult or impossible to navigate once interaction begins. Yet, most automated accessibility checkers miss failures involving focus, interface state, and accessible feedback across interactions. We present A11yLTLNav, a property-based approach for automatically detecting accessibility navigation failures. Through a structured review of prior research, we organize accessibility navigation failures into a failure taxonomy and formalize a browser-observable subset as executable Linear Temporal Logic properties over action-state traces. A11yLTLNav combines random keyboard exploration with runtime property monitoring to detect these failures during interactions. We evaluate A11yLTLNav on 31 generated websites based on real-world websites and tasks. It reported 309 accessibility failures, of which 274 were confirmed, achieving 88.7% precision and identifying more confirmed failures than the comparison checkers. Our results show that A11yLTLNav transforms accessibility knowledge into reusable checks of interface behavior over time.

==> unformalized_failure_rationale.tex <==
\subsection{Why some taxonomy failures are not yet executable}
\label{appendix:unformalized-failures}

Across the 35 failure categories in our taxonomy, the current property set
operationalizes 22 with at least one executable temporal property. The remaining
13 are not omitted because they are inexpressible in LTL. Rather, an executable
property must be grounded in predicates that the checker can observe and
attribute to a concrete interaction. For these failures, at least one required
predicate depends on information that is not available from browser state alone,
such as a semantic relation between interface regions, an operation lifecycle,
assistive-technology behavior, a task or relevance oracle, a calibrated cost
threshold, or persistent cross-view identity. Table~\ref{tab:unformalized-taxonomy}
summarizes these boundaries and the additional support that would be needed to
encode them as Bombadil properties.

\begingroup
\footnotesize
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{1.14}
\begin{longtable}{@{}>{\centering\arraybackslash}p{1.0cm}
                        >{\RaggedRight\arraybackslash}p{4.1cm}
                        >{\RaggedRight\arraybackslash}p{4.8cm}
                        >{\RaggedRight\arraybackslash}p{4.5cm}@{}}
\caption{Taxonomy failures not directly formalized by the current browser-observable property set. These failures are not necessarily inexpressible in LTL; the limitation is that one or more predicates needed for an executable check are not currently grounded by Bombadil.}
\label{tab:unformalized-taxonomy}\\
\toprule
\textbf{Level} & \textbf{Failure} & \textbf{Why it is not directly executable} & \textbf{Additional Bombadil support needed}\\
\midrule
\endfirsthead

\multicolumn{4}{@{}l}{\footnotesize\itshape Table~\ref{tab:unformalized-taxonomy}, continued}\\[1pt]
\toprule
\textbf{Level} & \textbf{Failure} & \textbf{Why it is not directly executable} & \textbf{Additional Bombadil support needed}\\
\midrule
\endhead

\midrule
\multicolumn{4}{r@{}}{\footnotesize\itshape continued on the next page}\\
\endfoot

\bottomrule
\endlastfoot

\texttt{L2}
& Misplaced or disconnected response to an activation
& A state change can be observed, but browser state alone does not establish which region is the semantically intended response to the triggering control.
& A declared or inferred trigger-to-response-region relation that binds the activated control to the region expected to change.\\
\addlinespace[1.2pt]

\texttt{L2}
& Inadequate labels to reveal nearby context
& The checker can observe a label and surrounding elements, but it cannot infer which nearby context is necessary for the label to be meaningful.
& An element-to-context relation or semantic oracle specifying which surrounding information is required for interpretation.\\
\addlinespace[1.2pt]

\texttt{L2}
& No trace of operation progress or mode
& Checking progress or mode requires knowing when an operation starts, remains active, changes phase, and completes; those lifecycle boundaries are not generally exposed by the page.
& An operation or mode lifecycle recorder with explicit start, progress, completion, and cancellation states.\\
\addlinespace[1.2pt]

\texttt{L2}
& No reachable control to stop auto-playing media
& The checker may observe media and controls independently, but it cannot reliably determine which control stops the exact auto-playing media instance.
& A media-to-control binding plus a reachability check for the identified stop or pause control.\\
\addlinespace[1.2pt]

\texttt{L2}
& Inconsistent name exposure across reading modes
& DOM and ARIA state do not establish how a screen reader exposes the same element in browse mode versus forms or focus mode.
& Assistive-technology-level observations aligned with screen-reader mode and browser focus.\\
\addlinespace[1.2pt]

\texttt{L2}
& Screen-reader shortcut captured outside the page
& A failed shortcut may be handled by the page, browser, operating system, extension, accessibility widget, or screen reader; browser-level evidence cannot reliably attribute the capture.
& OS- and assistive-technology-level key-event tracing that identifies which component consumed the shortcut.\\
\addlinespace[1.2pt]

\texttt{L3}
& Inadequate description of goal-relevant information
& Whether an existing description is sufficient depends on what information the user's task requires, not only on whether the description is present.
& A task or relevance oracle that represents the user's information goal and judges whether the exposed description supports it.\\
\addlinespace[1.2pt]

\texttt{L3}
& Reading order and grouping inconsistent with the task's logic
& The browser exposes document order and grouping, but the checker does not know the task-dependent relationships that should determine the useful order or grouping.
& A task model that specifies relevant objects, relationships, and expected grouping or ordering.\\
\addlinespace[1.2pt]

\texttt{L3}
& Excessive heading marks relative to page content
& Heading density is observable, but there is no task-independent threshold at which the number of headings becomes excessive for navigation.
& A calibrated density or navigation-cost threshold, potentially conditioned on page structure or task context.\\
\addlinespace[1.2pt]

\texttt{L3}
& Tab order inconsistent with the task's order
& The actual Tab sequence is observable, but the checker has no general oracle for the order in which controls should be encountered for a particular goal.
& A declared task order or task-derived partial order over relevant controls.\\
\addlinespace[1.2pt]

\texttt{L3}
& No efficient route to the control the task requires
& Efficiency requires both knowing the task-relevant target and deciding how much navigation cost is acceptable; neither is defined by browser state alone.
& A task-target oracle together with a navigation-cost model or explicit cost bound.\\
\addlinespace[1.2pt]

\texttt{L3}
& No confirmation of completeness, driving re-verification
& The checker cannot infer when the user has seen enough task-relevant evidence to know that a review or search is complete.
& A task-completion model that represents relevant evidence and the conditions under which completeness can be established.\\
\addlinespace[1.2pt]

\texttt{L3}
& No means of resuming from a prior position
& Checking resumption requires a stable identity for the user's prior interaction position across navigation or re-rendering and a definition of equivalent restoration.
& Persistent cross-view position identity and history tracking that can compare the restored location with the prior task position.\\

\end{longtable}
\endgroup

The 22 mapped failure categories should therefore be interpreted as coverage by
at least one executable property, not as exhaustive coverage of every instance
of that category. Several implemented properties intentionally capture narrower,
high-confidence subtypes for which the trigger and expected outcome can be
observed reliably in the browser. This conservative boundary keeps the LTL
specification aligned with what the Bombadil monitor can actually establish from
an execution trace.

